RankFeat: Rank-1 Feature Removal for Out-of-distribution Detection

The task of out-of-distribution (OOD) detection is crucial for deploying machine learning models in real-world settings. In this paper, we observe that the singular value distributions of the in-distribution (ID) and OOD features are quite different: the OOD feature matrix tends to have a larger dominant singular value than the ID feature, and the class predictions of OOD samples are largely determined by it. This observation motivates us to propose \texttt{RankFeat}, a simple yet effective \texttt{post hoc} approach for OOD detection by removing the rank-1 matrix composed of the largest singular value and the associated singular vectors from the high-level feature (\emph{i.e.,} $\mathbf{X}{-} \mathbf{s}_{1}\mathbf{u}_{1}\mathbf{v}_{1}^{T}$). \texttt{RankFeat} achieves the \emph{state-of-the-art} performance and reduces the average false positive rate (FPR95) by 17.90\% compared with the previous best method. Extensive ablation studies and comprehensive theoretical analyses are presented to support the empirical results.

==> AC_letter.tex <==
Dear ACs and senior ACs,

  We are not really convinced by the rationale behind the scores of $\color{brown}{Reviewer\ SMeo\ (R4)}$ and $\color{blue}{Reviewer\ dq6u\ (R2)}$ though we fully respect their decisions.
    
  $\color{blue}{R2}$ argued that field of *post hoc* OOD detection makes little sense and should not be different from training-needed OOD detection, which we strongly disagree. $\color{blue}{R2}$ seems to have prejudices against *post hoc* OOD detection and his argument is denying this research direction, but actually there are many *post hoc* OOD approaches [1,2,3] proposed recently. Compared with training-needed methods, *post hoc* approaches have the benefit of ***(1)*** *direct application to any pre-trained models*, ***(2)*** *easy use due to widely available pre-trained models*, ***(3)*** *no interference on the standard ID classification accuracy*, and ***(4)*** *application in scenarios where training data are not available*. Moreover, for the comparison of *post hoc* methods against training-needed approaches (as requested and insisted by $\color{blue}{R2}$), the additional training procedure and extra usage of training data of training-needed approaches are very unfair to *post hoc* approaches. We have shown that given extra training, *post hoc* methods can also have very competitive performance. Furthermore, $\color{blue}{R2}$ has made many obvious mistakes throughout the replies: ***(1)*** *$\color{blue}{R2}$ mistakenly argues our method need extra training.* ***(2)*** *$\color{blue}{R2}$ wrongly uses Figure 3 of PANDA [4] to show the performance* ***(3)*** *$\color{blue}{R2}$ mistakenly argues that our method incurs huge time consumption*. Last but not the least, we feel that $\color{blue}{R2}$ seems to intentionally neglect the crucial points but selectively replying to the minor points, especially in the latest few responses. 
  
  %He/she also thinks that CIFAR benchmark is more critical than ImageNet-1k benchmark. 

  $\color{brown}{R4}$ insisted that there should be a strong theoretical guarantee that can prove our observation holds for every benchmark and every model, and empirical evidence on several benchmark is not sufficient. However, how to give strong theoretical guarantee for *post hoc* OOD method is an open problem. To the best of our knowledge, no prior work could give a strong score guarantee [1,2,3], and most of them are also based on empirical and intuitive observations. For our method, our observation is supported by ***(1)*** *empirical results on several benchmarks*, ***(2)*** *visualization of singular value distributions*, and ***(3)*** *PCA-based informativeness explanations*. We believe that these evidences should be sufficient to support our opinion. Also, we noticed that $\color{brown}{R4}$ has secretly lowered the score several times during the rebuttal phase without any notification or justification. On Friday (05/08/2022), he/she secretly decreased the score from 5 to 4 during the discussion. On Sunday (07/08/2022), he/she secretly decreased the score from 6 to 5 again two days after our final discussion. Moreover, throughout the replies, he/she promised "I will increase your score to 7" several times and promised "I will increase your score to 6." in the latest reply but failed to do so after we addressed the issues. Although we respect that $\color{brown}{R4}$ has the right to change the score as he/she likes, we are not convinced by so frequent & uninformed changes and un-aboveboard & inconsistent actions. 
  
Best regards,

Authors
  
>[1] Energy-based Out-of-distribution Detection. NeurIPS 2020
>
>[2] ReAct: Out-of-distribution Detection With Rectified Activations. NeurIPS 2021
>
>[3] On the Importance of Gradients for Detecting Distributional Shifts in the Wild. NeurIPS 2021
>
>[4] Panda: Adapting pretrained features for anomaly detection and segmentation. CVPR 2021
